Some algebraic identity and its relations to Stirling numbers of the second kind

In this short note we provide some algebraic identity with a proof exploiting its probabilistic interpretation. We show several consequences of the identity, in particular we obtain a new representation of a Stirling number of second kind, $$ S(n,d)={1\over d!} \sum_{1\leq j_1<j_2<\ldots<j_{d-1}< n} 1\cdot2^{j_{d-1}-j_{d-2}}\cdots d^{j_1}$$ for integers $n\geq d$. Relating this to other known formula for $S(n,d)$ we also obtain $$ \sum_{1\leq j_1\leq j_2\leq \cdots\leq j_{n-d}\leq d} j_1j_2\ldots,j_{n-d} =d! \sum_{1\leq j_1<j_2<\ldots<j_{d-1}< n} 1\cdot2^{j_{d-1}-j_{d-2}}\cdots d^{j_1}.$$ As a side effect, we have new proof of a known result stating that for any integer $d\in\mathbb{N}$ and any $x\in\mathbb{R}$ equality $$\sum_{r=0}^d (-1)^r{d\choose r}(x-r)^d=d!$$ holds. This is a special case of the presented identity.

==> setup/alg.tex <==
% !TEX root = ../main.tex
% = = = Framed Boxes (Construction, Protocol)
%\usepackage{framed}
\usepackage{float}
\newfloat{Protocol}{t}{struct}

% = = = Use:

%\begin{Protocol*}[t!]
%\begin{framed}
%\textbf{Title}\\
%\footnotesize
%
%	content
%
%\normalsize	
%\end{framed}
%\caption{Caption and stuff\label{alg:lab}}
%\end{Protocol*}

==> setup/macros.tex <==
% !TEX root = ../main.tex
%------------------------Custom Commands----------------------%

% = = = Latin Short-forms (ie, eg, etc, et al)
\usepackage{xspace}
\newcommand{\etal}{\textit{et al.}\xspace}
\newcommand{\etc}{\textit{etc.}\xspace}
\newcommand{\ie}{\textit{i.e.,}\xspace}
\newcommand{\eg}{\textit{e.g.,}\xspace}
\newcommand{\cf}{\textit{cf.}\xspace}
\newcommand{\supra}{\textit{Supra}\xspace}

% = = = Arrow -> (\lt)
\newcommand{\lt}{$\rightarrow$\xspace}

% = = = Keywords (kw)
\newcommand{\kw}[1]{\textsf{#1}}

% = = = Colored text (textblue)
\newcommand{\textblue}[1]{\textcolor{blue}{#1}}

% = = = Compact Lists (compactlist, compactlistn)
\newenvironment{compactlist}
  {\begin{itemize} 
  \setlength{\itemsep}{0pt} 
  \setlength{\parskip}{0pt}} 
  {\end{itemize}}
  
\newenvironment{compactlistn}
  {\begin{enumerate} 
  \setlength{\itemsep}{0pt} 
  \setlength{\parskip}{0pt}} 
  {\end{enumerate}}
  
\renewcommand{\labelitemi}{$\bullet$}
  
  
  %peyo:
  \newcommand{\PP}[0]{\mathbf{P}}
  \newcommand{\indic}[0]{\mathds{1}}
%  \newcommand{\E}[0]{\mathbb{E}}
%------------------------Crypto----------------------%  

% = = = Zp, Gq and Zq
\newcommand{\Zp}{\mathbb{Z}^{*}_{p}}
\newcommand{\Zq}{\mathbb{Z}_{q}}
\newcommand{\Gq}{\mathbb{G}_{q}}
\newcommand{\E}[0]{\mathbb{E}}
\newcommand{\R}[0]{\mathbb R}
\newcommand{\RR6}[0]{\mathbb RR}

\newcommand{\x}[0]{\mathbf{x}}
\newcommand{\s}[0]{\mathbf{s}}
\newcommand{\C}[0]{\mathbf{C}}
\newcommand{\X}[0]{\mathbf{X}}
\newcommand{\Z}[0]{\mathbf{Z}}
\newcommand{\p}[0]{\mathbf{p}}
\newcommand{\q}[0]{\mathbf{q}}




% = = = Encryption, etc.
\newcommand{\Enc}[1]{\mathsf{Enc}(#1)}
\newcommand{\EncB}[1]{\llbracket #1 \rrbracket}
\newcommand{\ReRand}[1]{\mathsf{ReRand}(#1)}
\newcommand{\Hash}[1]{\mathcal{H}(#1)}
\newcommand{\Sign}[1]{\mathsf{Sig}(#1)}
\newcommand{\Comm}[1]{\mathsf{Comm}(#1)}
\newcommand{\Open}[1]{\mathsf{Open}(#1)}
\newcommand{\PRG}[1]{\mathsf{PRG}(#1)}

% = = = Tuples
\newcommand{\tuple}[1]{\left \langle #1 \right \rangle}


%-------------------Custom for Paper----------------------%

% = = = Name
\newcommand{\ballotid}{\textsf{VoteSerial}\xspace}
\newcommand{\code}{\textsf{VoteCode}\xspace}

\newcommand{\serial}{\textsf{AuthSerial}\xspace}
\newcommand{\auth}{\textsf{AuthCode}\xspace}
\newcommand{\ack}{\textsf{AckCode}\xspace}
\newcommand{\sig}{\textsf{Sig}(\%)\xspace}
\newcommand{\lock}{\textsf{LockCode}\xspace}


\definecolor{ltgray}{RGB}{200,200,200}
\definecolor{dkgray}{RGB}{150,150,150}
\newcommand{\scratch}[1]{\fcolorbox{dkgray}{ltgray}{$#1$}\xspace}




==> setup/packages.tex <==
% !TEX root = ../main.tex

%------------------------LNCS----------------------%

%------------------------Packages----------------------%

% = = = Graphics
% \usepackage[pdftex]{graphicx}
% \graphicspath{{figures/}}
% \DeclareGraphicsExtensions{.jpg,.png}


% = = = Subfig (note not subfigure)
% \usepackage[caption=false,font=footnotesize]{subfig}

% = = = Math Symbols
% \usepackage[cmex10]{amsmath}
% \usepackage{bbm,stmaryrd}

% = = = Other
\usepackage{array}
\usepackage{color}
%\usepackage[hyphens]{url}
%\usepackage{multirow}
% \usepackage[pdftitle=Remotegrity,pdfauthor=Anonymous]{hyperref}

%------------------------END----------------------%  
  

%\documentclass[a4paper,8pt]{article}

\usepackage{epsfig}
\usepackage{amssymb}
\usepackage{graphicx}
\usepackage{fancyhdr}

\usepackage{algorithm}
\usepackage{algorithmic}
%\usepackage{algpseudocode}
%\usepackage[noend]{algpseudocode}


%\usepackage{pstricks}
 

% \usepackage[colorlinks = true,
%             linkcolor = blue,
%             %urlcolor  = magenta,
%             urlcolor = blue,
%             %urlcolor  = burntorange,
%             %urlcolor =  tangerine,
%             citecolor = blue,
%             anchorcolor = blue]{hyperref}
            
\usepackage{amsthm}
\usepackage{amsmath}
% \newtheorem{deff}{Definition}[section]
% \newtheorem{twr}[deff]{Theorem}
% %\newtheorem{theorem}{Theorem}
% %\newtheorem{example}{Example}
% %\newtheorem{corr}{Corrolary}
% \newtheorem{lem}[deff]{Lemma}
% \newtheorem{fact}[deff]{Fact}
% \newtheorem{prop}[deff]{Proposition}
% \newtheorem{uwaga}[deff]{Remark}
% \newtheorem{alg}[deff]{Algorithm}
% \newtheorem{wniosek}[deff]{Conclusion}

%\newcommand{\comment}[1]{}

% \renewcommand\theequation{\arabic{equation}}
% \newcommand{\e}[0]{\mathbf{e}}
% \newcommand{\PP}[0]{\mathbf{P}}
% \newcommand{\KK}[0]{\mathbf{K}}
% \newcommand{\Q}[0]{\mathbf{Q}}
% \newcommand{\E}[0]{\mathbb{E}}
% \newcommand{\s}[0]{\mathbf{s}}

%\newcounter{licznik2}
%\renewcommand\theequation{\arabic{equation}}

\addtolength{\voffset}{-2.5cm}
%\addtolength{\textheight}{5.5cm}



\setlength{\parindent}{0cm}

%odst w tabl, ale nie dziala
%\setlength{\tabcolsep}{3cm}

\addtolength{\hoffset}{-1cm}
\addtolength{\textwidth}{2.0cm}

\pagestyle{fancy}
\renewcommand\headrulewidth{0pt}
\fancyhead[LE,LO,RE,RO]{}
\fancyfoot[LE,LO]{\tiny {\tt\jobname  }}
\fancyfoot[RE,RO]{\tiny {\tt \leftmark     }}
%\rightmark - \leftmark --
\fancyfoot[c]{\thepage  }

\usepackage{dsfont}
